Tensor Embedding: A Supervised Framework for Human Behavioral Data Mining and Prediction

Today's densely instrumented world offers tremendous opportunities for continuous acquisition and analysis of multimodal sensor data providing temporal characterization of an individual's behaviors. Is it possible to efficiently couple such rich sensor data with predictive modeling techniques to provide contextual, and insightful assessments of individual performance and wellbeing? Prediction of different aspects of human behavior from these noisy, incomplete, and heterogeneous bio-behavioral temporal data is a challenging problem, beyond unsupervised discovery of latent structures. We propose a Supervised Tensor Embedding (STE) algorithm for high dimension multimodal data with join decomposition of input and target variable. Furthermore, we show that features selection will help to reduce the contamination in the prediction and increase the performance. The efficiently of the methods was tested via two different real world datasets.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios
		Code prettying (Michael D. Adams)
		Two-column formats now balance the last page (ACM request)
		

==> image/main_body.tex <==
\section{Introduction}

The rapid growth in technology, has increased the opportunity for longitudinal human behavioral studies \cite{miluzzo2008sensing,bang2008toward,aldwin2007stress,StudentLife2014,choudhury2008mobile}. Today's densely instrumented world offers tremendous opportunities for continuous acquisition and analysis of multi-variant time series data that provides a multimodal characterization of an individual's actions. 

Integrating different sensor technologies to enable continuous, unobtrusive sensing of individual physiological states, their activity, and their environmental and social contexts is challenging. There have been several studies collected multimodal in real-world. StudentLife is a 10-week study on 48 Dartmouth undergraduate and graduate students using passive and mobile sensor data to infer wellbeing, academic performance and behavioral trends \cite{StudentLife2014}. The Dartmouth College research team was able to predict GPA using activity, conversational interaction, mobility, and self-reported emotion and stress data over the semester. SNAPSHOT is a 30-day study on MIT undergraduates using mobile sensors and surveys to understand sleep, social interactions, affect, performance, stress and health \cite{3-2}. RealityMining is a 9-month study on 75 MIT Media Laboratory students, using mobile sensor data to track the social interactions and networkings \cite{3-3}. The friends-and-families study collects data from 130 adult members of a young family community to study fitness intervention and social incentives \cite{aharony2011social}. We designed an experiment to examine the complex interplay between individual differences, job performance, and well-being with varying cognitive, affective and social demands. More than 200 nurses were instrumented with different sensors during their work shift for a duration of 1 to 2 months.

The next challenge in these type of studies would be how to fuse noisy, incomplete, and heterogeneous bio-behavioral data from sensors operating in different modalities and temporal resolution scales, and to extract features for analysis and predictive purposes. All these data sources are often collected from small set of participants in natural condition, continuously and over long periods of time. Therefore, they are potentially heterogeneous, sparse, in high dimensional regime and have systematically missing values. Aggregating the data over the time dimension, or matricizing the tensor, Partial Least Squares (PLS) regression \cite{pls} and Principal Component Analysis (PCA) \cite{20} would particularly appropriate for these high dimension tasks. While PCA find the direction with highest variation, independent of dependent variable, PLS considers both the independent and dependent variables by projecting them to the low dimensional latent variables space. For the purpose of interpretability, we are looking for techniques such as higher order PCA and PLS which can be applied directly to N-way data. We are interested in prediction of a certain set of behaviors from these multi-way data. Latent user factor matrix obtained from unsupervised tensor decomposition approaches can be used as the extracted features with any conventional regression method. However, there is no guarantee these new features, however there is no guarantee for having any predictability power for the target variable of interest. We are interested in supervised embedding technique to overcome this challenge. Previously \cite{hoff2015multilinear} has looked at tensor regression problem for relational longitudinal data. \cite{Tao2007Supervised} supervised tensor learning for classification problem, extended SVM and MPM. With join CP decomposition of input and target variable, NPLS is one of the widely used methods for higher order regression problems, \cite{}. \cite{zhao2013higher} improve the predictability performance and \cite{hou2017fast} make it faster for large scale data with developing a sequential low-rank tensor regression framework. Several works later work on the scalability and speed of HOPLS \cite{}. HOPLS was designed for Y with number of dimension more than 1. We are the most similar to NPLS, as the analysis of NPLS weights and NPLS regression coefficients allows data patterns, feature correlation and covariance structure to be depicted. Later \cite{favilla2013assessing} propose an extension of the Variable Importance in Projection (VIP) parameter to multi-way arrays in order to highlight the most relevant features to predict the studied dependent variable and have presented examples for interpretative purposes. 
 
Here we propose a supervised embedding to latent space, which find the weights of latent components for all three dimensions similar to NPLS. We also combine it with variable selection by using the component activation power. We can then use any linear or non-linear regression function for the prediction task. The framework for our method is depicted in Figure \ref{fig:workflow}. Basically we first use covariance matrix of input and target variable and find the feature importance vector, and then we select the top K important features and apply supervised factorization in reduced sized tensor.  

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.65\textwidth]{image/model.png}
    \caption{Framework from tensor $X$ to prediction $\hat{y}$.}
    \label{fig:workflow}
\end{figure*}

\subsection*{Contributions}
\begin{itemize}
\item A large-scale "in the wild" experimental studies that collect bio-behavioral data from subjects who are facing challenging cognitive, social, and affective demands in their natural settings.
  \item Proposed a tensor-input/vector-output Recursive Tensor Embedding (STE) algorithm for high dimension multi-way (tensor) noisy data
  \item Variable selection using components' activation is united with supervised embedding 
  \item Validation of recovered latent patterns via prediction performance over synthetic data and two real world datasets 
  
\end{itemize}

\section{Data Collection}

Tracking Individual Performance with Sensors study, tracks nurses performance, wellbeing and physiological state for duration of 2 months. We developed a smartphone application called TILES for collecting data from more than 200 nurses during their work shift. It is a 4-week study conducted during spring and summer 2018 on 201 nurses. The dataset can be divided into four sections: sensory data, health variables, psychometrics and job performances. Sensory data includes HRV metrics collected via OM sensors, Fitbit collects Hear rate and steps. 


Psychometrics have pre-surveys of Big Five personality \cite{2-2}, positive and negative affect schedule (PANAS) \cite{2-8}, Pittsburgh sleep quality index (PSQI) \cite{2-5} and ... . 

\section{Methodology}

\subsection{Notation and definitions}
A wide range of real-world datasets are multi-way, e.g. in neuroscience \cite{1}, complex networks \cite{2}, social networks \cite{2}, etc. A mathematical representation of such data is tensor, $\mathcal{X} \in \mathbb{R}^{I_1 \times ... \times I_N}$, when element ($i_1,i_2,...,i_N$) of an $N$th (number of dimensions) order tensor  is denoted by $x_{i_1}$ . Table \ref{tab:notation} provides a summary of the notations. In this work we are dealing with temporal data, presented in terms of 3-way tensors. 
 
 
 NPLS is higher order PLS regression which preserves the structure of the data by avoiding vectorization of the data. For independent and dependent tensors of observation $ \mathcal{X} \in \mathbb{R}^{I \times J \times K}$ and $Y \in  I \times 1 $, the NPLS iteratively constructs the linear relationship by projecting them to the space of latent variables similar to the PLS way. In this section we discuss the model that we will use to analyze a 3-way longitudinal human behavioral data. For $I$ individuals, with $J$ variables for a duration of $K$ time frames, tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K } $ will be created. Entry $x_{ijk}$ of this tensor corresponds to the $i^{th}$ person in the $j^{th}$ variable at the $k^{th}$ time unit. Table \ref{tab:notation} summarizes our notation throughout this paper. 
 


Ordinary Partial Least Squares regression \cite{pls} is an iterative procedure to estimate a linear relationship between a vector of independent (input) variables and a vector of dependent (output) variables on the basis of observation matrices $X \in  N \times n$ and $Y \in  N \times m : Y = XB + D$ , where $B \in  n \times m$ is the matrix of linear coefficients, and $D \in  N \times m$ is the matrix of noise. To build the model, the observations are iteratively projected into the low dimensional spaces of latent variables while trying to explain the maximum of variance of $X$ and $Y$ simultaneously: $X = TP^T + E$ , $Y = UQ^T + F$; where $T = [t_1 , … , t_R ] \in   N \times F$ and $U = [u_1 , … , u_R ] \in  N \times F$ are the matrices of the latent variables (scores), $P = [p_1 , … , p_R ] \in  n \times R$ and $Q = [q_1 , … , q_R ] \in  m \times R$ are the matrices of the loading vectors (projectors), E and F are residual matrices, and F is the number of iterations (factors). The PLS approach is particularly well suited for high dimensional data due to its efficient dimensional reduction technique. Multi-way Partial Least Squares (NPLS) regression is an algorithm in the PLS-family that is adopted to the case of tensor variables \cite{npla}.



 



\begin{table}
	\centering
    \caption{Table of Symbols.}
	\begin{tabular}{c|c}
	\hline \hline
	Symbol & Definition \\ \hline
	\hline
    $\mathcal{X},\mathrm{X},\mathbf{x},\mathrm{x}$ & Tensor, matrix, column vector, scaler\\ \hline
	$ \mathbf{x} \in \mathbb{R}^{I\times 1} $ & Definition of an I-dimensional vector  \\	\hline
     $\circ$  & Outer product \\\hline
    $||.||$ & Frobenius norm \\ \hline \hline
	\end{tabular}
	
	\label{tab:notation}  
\end{table}

\subsection{Variable Selection}

\subsection{supervised tensor decomposition}
  The extraction of meaningful patterns of behavior can be carried out by taking full advantage of tensor decomposition techniques. Let us consider a dataset composed by individuals, whose daily behavior (walking, running, talking, etc. during the day)  has been recorded over time. To uncover groups of individuals with similar correlated trajectories, identification of lower-dimensional factors is required. Once the dataset is represented in the tensor form, we can perform tensor decomposition to discover the hidden lower dimension structure of the data. 


Here, we use the CANDECOMP/PARAFAC decomposition \cite{carroll1970analysis,harshman1970foundations}, which will decompose the tensor $\mathcal{X} \in R^{I \times J \times K}$ into sum of rank-one tensors, called components, Figure \ref{fig:cp}. Also we add the non-negativity constraints to each factor matrix in order to find interpretable components.


% = [\![\mathrm{U},\mathrm{V},\mathrm{T}]\!]

\begin{align*}
\mathcal{X} \approx \hat{\mathcal{X} } =  \sum_{r=1}^{R} \lambda_r \mathbf{u}_r \circ \mathbf{v}_r \circ \mathbf{t}_r 
\end{align*}


where $\lambda_r$ are the values of the tensor core $L = diag(\Lambda)$, and the outer product $\mathbf{u}_r~o~\mathbf{v}_r~o~\mathbf{t}_r$ corresponds to the $r^{th}$ component of rank-R estimation.  



$\mathbf{U}, \mathrm{V}, \mathrm{T}$ are the factor matrices with their columns containing rank-1 factors, $\mathbf{u}_r, \mathbf{v}_r$, and $\mathbf{t}_r$, respectively. Imposing the non-negativity constraints makes the factorization results interpretable. 

%Share decomposition of different matrices can be translated into decomposition of a tensor. 

I the simulations, STE, and NPLS were used to model the data in a tensor form, when PLS is used on a mode-1 matricized version of the same tensor. To compare the predictability, we compare root mean square error (RMSE), coefficient of determination $R^2$ and pearson correlation $\rho$.  \ref{alg:euclid}

\subsection{Supervised Tensor Embedding}


\begin{algorithm}
\caption{Supervised Tensor Embedding}\label{alg:STE}
\begin{algorithmic}[1]
\State input: $\mathcal{X}$ independent tensor, $y$ dependent variable
\State parameters: $R$ - decomposition rank
\State output: $U,T,V$  
\State Center $\mathcal{X}$ and $\mathbf{y}$
\State ${\mathcal{X}}_{rem} = \mathcal{X}$
\For{r = 1:R}
\State Calculate $Z = COV<\mathcal{X}_{rem},\mathbf{y}>$
\State $\mathbf{t}_r,\mathbf{v}_r \leftarrow SVD(Z)$ 
\State $\mathbf{u} \leftarrow \mathbf{t},\mathbf{v}$ 
\State $\mathbf{X_{R=1}} \leftarrow \mathbf{t},\mathbf{v}$ 
\State $\mathcal{X}_{rem} = \mathcal{X}_{rem} - \mathcal{X}$ 
\EndFor
\end{algorithmic}
\end{algorithm}

\subsection{Variable Selection}


For variable selection we take the latent factor matrix V and extract the variable importance as following:

\begin{equation*}
FI_i = \sum_{r=1}^{R} \mathbf{v}^2_{ri}
\end{equation*}

\subsection{Regression model}


\begin{algorithm}
\caption{Supervised Tensor Embedding with Time Series Selection}\label{alg:STE}
\begin{algorithmic}[1]
\State input: $\mathcal{X}$ independent tensor, $y$ dependent variable
\State parameters: $K$ - number of variables, $R$ - decomposition rank , f()- regression function
\State output: $\hat{y}$  
\State Compute component activation for each sensory variable using alg1
\State Form a reduced data tensor consisting of only time series whose activation power is among top K variables
\State Compute latent variables using alg2 
\State Use latent variables in a regression model to predict outcome $\hat{y} = f(U)$
\State Pick K and parameter of model $f(.)$ by cross validation 
\end{algorithmic}
\end{algorithm}
\section{Experimental result}
I the simulations, STE, and NPLS were used to model the data in a tensor form, when PLS is was used on a mode-1 matricized version of the same tensor. To compare the predictability, we compare root mean square error (RMSE), coefficient of determination $R^2$ and and spearman correlation $\rho$.  	

\subsection{Synthetic data}
To quantitatively benchmark our algorithm, an extensive comparative exploration has been performed on synthetic datasets to evaluate the prediction performance under different conditions with respect to data structure, noise levels, correlation between features. For parameter selection, the number of latent vectors (R) and number of selected variables (K) were chosen based on cross-validation. To reduce random fluctuations, evaluations were performed over 50 validation datasets generated repeatedly according to the same criteria.

To construct the input tensors and target vectors, random factor matrices with entries following standard normal distribution are generated and a tensor is formed based on a CP model. We generate random factor matrices $U \in R^{N \times R}$ , $T \in R^{I \times R}$ and $V \in R^{J \times R}$ , and form a third-order tensor $\mathcal{X} \in R^{N \times I \times J}$ based on a CP model. Gaussian noise is later added to the tensor, i.e., $\mathcal{X} \in R^{N \times I \times J}$, where $\mathcal{X} \in R^{N \times I \times J}$ responds to the random noise tensor and $\eta$ is used to adjust the noise level. Similarly, we generate a factor matrix $\mathcal{X} \in R^{N \times I \times J}$ and form vector $\mathcal{X} \in R^{N \times I \times J}$ . The matrix $N \in R^{I \times R}$ is a matrix with entries drawn from the standard normal distribution and is used to introduce differing amounts of noise in the data. In our experiments, we use three different noise levels, i.e., $\eta$ = 0.1, 0.25 and 0.35, and the true number of factors is $R$ = 3. \ref{meshplots}



\begin{figure}[h]
\label{meshplots}
\centering
\begin{subfigure}{.25\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{image/romesh9db.png}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{image/romesh3db.png}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{image/romesh6db.png}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{image/romesh9db.png}
\end{subfigure}
\caption{Held-out performance of STE at different noise levels versus the number of latent variables (R) and number of selected variables (K). (-9db: $\lambda=0.5$, -9db: $\lambda=0.5$,-9db: $\lambda=0.5$,-9db: $\lambda=0.5$}
\end{figure}

\subsection{Real data}
Our goal in this paper is understanding whether using supervised decomposition we can find the low-dimensional structure of daily life from wearable devices, which correlated with self-reported target variables better than unsupervised decomposition. We test our model on two real world datasets, TILES ans StudentLife.




\subsubsection*{TILES}
     We will use the pre-survey scores as dependent variables. Each time unit comprise one day worth of data, and is divided into four time bins, bedtime (midnight-6 am), morning (6 am-12 pm), afternoon (12 pm-6 pm), and evening (6 pm-midnight). We extract a set of statistics such as mean, standard deviation, kurtosis, etc. from each times series from OMSignal and Fitbit, in each time bin. At the end, we organize our data as tensor $\mathcal{X}$ with $I=200$ individuals, $J=650$ variables and $K=31$ days. Only x\% of the tensor is missing, which we imputed by filling them with the mean value. 
    
\subsubsection*{StudentLife}
StudentLife is a 10-week study conducted during 2013 spring semester on 48 Dartmouth students (30 undergraduate and 18 graduate students). From raw sensory data, activity (stationary, walk, run and unknown), audio (silence, voice, noise and unknown), and conversation has been inferred. Each time unit comprise one day worth of data, and is divided into four time bins, bedtime (midnight-6 am), morning (6 am-12 pm), afternoon (12 pm-6 pm), and evening (6 pm-midnight). We extract duration (minutes) of running, walking, stationary, silence, voice, noise, and dark, per time-bin in each day. Frequency of each behavior and number of changes in each behavior (e.g. from walking to running) for each time-bin has been also captured. From GPS and WiFi, number of unique locations visited, and from Bluetooth number of unique near by devices per time-bin are added to the variable set. We normalize all the variables to have the same range $[0,1]$ to avoid variables with large values (e.g. duration in minutes) dominate the analysis. At the end, we organize our data as tensor $\mathcal{X}$ with $I=48$ individuals, $J=85$ variables and $K=66$ days. Only 5\% of the tensor is missing, which we imputed by filling them with the mean value. 

\subsection*{Results}

We tested our model for 20 different target variables with basic NPLS and STE with variable selection. 

\begin{table*}
\begin{center}
\caption{Personality traits prediction}
 \begin{tabular}{||c |  c | c | c | c | c ||} 
 \hline
   & Agreeableness & Openness & Conscientiousness & Extraversion & Neuroticism\\ [0.5ex] 
 \hline\hline
 $ \rho$ &   &   &   & &  \\ 
 \hline
$R^{2}$ &   &   &   & & \\
 \hline
 \hline
 $ \rho$ - NPLS&   &   &   & &  \\ 
 \hline
$R^{2}$ - NPLS&   &   &   & & \\
 \hline
\end{tabular}
\end{center}
\label{personality}
\end{table*}

\begin{table*}
\begin{center}
\caption{Job performance and cognitive abilitys prediction}
 \begin{tabular}{||c |  c | c | c | c | c | c | c ||} 
 \hline
   & ITP & IRB & IOD-ID & IOD-OD & OCB & Shipley abstract & Shipely vocabulary\\ [0.5ex] 
 \hline\hline
 $R^{2}$ &   &   &   & & & &  \\ 
 \hline
$\rho$ &   &   &   & & & & \\
 \hline
\end{tabular}
\end{center}
\label{job_cognitive}
\end{table*}


\begin{table*}
\begin{center}
\caption{TILES: Emotion and health variable prediction}
 \begin{tabular}{||c |  c | c | c | c | c | c ||} 
 \hline
   & Positive affect & Negative affect & Anxiety & Alchohol usage  & Excercise & Sleep quality\\ [0.5ex] 
 \hline\hline
 $R^{2}$ & 0.35 & 0.20 & 0.19 & 0.17 & 0.29& 0.06\\ 
 \hline
$\rho$ & 0.59 & 0.49 & 0.47 & 0.48& 0.54 & 0.23\\
 \hline
\end{tabular}
\end{center}
\label{emotion_health}
\end{table*}


\begin{table*}
\begin{center}
\caption{Student Life: performance and emotion}
 \begin{tabular}{||l | c |  c | c | c | c  ||} 
 \hline
   & GPA &  Stress &  Depression  & Florishing & Sleep quality\\ [0.5ex] 
 \hline\hline
  $\rho$& 0.54  &   0.40  & 0.39 & 0.32 &0.30 \\ 
 \hline
 $R^{2}$ & 0.29 R  & 0.16 & 0.12  & 0.10 RF &0.05 \\
 \hline  \hline
 $\rho$ - NPLS   & 0.40 & 0.47  & 0.31 & 0.23 &0.09 \\ 
 \hline
$R^{2}$ - NPLS  & 0.12 &   0.20 &  -0.01 & 0.02 &-0.14\\
 \hline
\end{tabular}
\end{center}
\label{emotion_health}
\end{table*}

\begin{table*}
\begin{center}
\caption{StudentLife: personality traits prediction}
 \begin{tabular}{||l |  c | c | c | c | c ||} 
 \hline
   & Agreeableness & Neuroticism  & Conscientiousness & Extraversion & Openness\\ [0.5ex] 
 \hline\hline
 $\rho$ & 0.43  & 0.48  & 0.56  & 0.45 & 0.49 \\ 
 \hline
$R^{2}$ & 0.06  & 0.21  & 0.31  & 0.20 & 0.19 \\
 \hline \hline
  $ \rho$ - NPLS & 0.09  & 0.33 & 0.40    &  0.13 & 0.33   \\ 
 \hline
$R^{2}$- NPLS  & -0.17  & 0.11 & 0.13     & 0.0 & -0.07   \\
 \hline
\end{tabular}
\end{center}
\label{personality}
\end{table*}

\subsection{Case study: Interpretability of the model}

\section{Conclusions and Future work}

Rich multimodal data collected from wearables devices (e.g. Fitbit), mobile phones, online social networks, etc. become increasingly available to reconstruct digital trails and study human behavior. In this paper, we adopt two real world datasets \textit{TILES} and \textit{StudentLife}, using passive and mobile sensors, with the goal of inferring wellbeing, performance, and personality.
We employ the supervised learning framework based on \textit{supervised tensor embedding} to find latent space highly correlated with target variable of interest. This type of decomposition can uncover latent user factors which are strong predictor of target variables. Further we explore how variable selection can improve the prediction performance and propose a robust variable selection frame work. Next, we plan to implement supervised predictions of individuals' performance and personality directly from different modalities, such as social media activity, location, audio.
	





